Optimal Control of Thin-Film Flow on a Flexible Topography

This work presents a mathematical model for the optimal control of thin-film flows over a flexible substrate influenced by an external force. The objective is to find the optimal distributed force acting on the topography that minimises the differences between actual and desired thin-film profiles. A nonlinear lubrication equation governing the fluid dynamics and appropriate functional settings for this model are presented. It is also shown that this system satisfies a global energy-dissipation law for a suitable energy functional. Optimality conditions are derived for the solution of the minimisation problem of a specified cost function across a time horizon. These conditions are formulated at a continuous level as system of coupled, forward-backward PDEs, which are subsequently discretised for numerical investigation. To ensure computational efficiency and stability, first-order Implicit-Explicit (IMEX) time-stepping schemes are employed to handle the nonlinearities in the model, and a reduced gradient descent algorithm is applied to obtain a numerical approximation of the optimal control signal. Numerical results illustrate that controlling the thin film, even during rupture, achieves a precise film profile. This control strategy accelerates convergence towards a steady state, reduces instabilities, stabilises dewetting processes, and meets the desired profile specifications.

==> 2-MATHEMATICAL_FORMULATION/Free_Energy.tex <==
\begin{equation}\begin{aligned}&\begin{aligned}& \left.\frac{d}{d t} \int\left[\phi(h)+\frac{1}{2 C_a} h_x^2+\frac{c^2}{2 \gamma} s_x^2+\frac{1}{C_a} h_x s_x\right]-\frac{B_o}{2 C_a} h^2\right] d t \\& =\int\left[\phi^{\prime}(h) h_t-\frac{1}{C_a} h_{x x}-\frac{B_o}{C_a} h h_t-\frac{c^2}{\gamma} s_x s_t+\frac{1}{C_a} \left(h_x s_x\right)_t\right].\end{aligned}\\&=\int[\underbrace{\phi^{\prime}(h)-\frac{1}{C_a} h_{x x}-\frac{B_o}{C_a} h}_{=\mu+\frac{1}{C_a} s_{x x}+\frac{B_o}{C_a} s}] h_t-\frac{1}{\gamma} \int c^2 s_{x x} s_t+\frac{1}{C_a} \int\left(h_x s_x\right)_t\\&\begin{aligned}=\int \mu h_t & +\int\left[\frac{1}{C_a} s_{x x}+\frac{B_o}{C_a} s\right] h_t-\frac{1}{\gamma} \int s_t^2+\int\left[\frac{1}{C_a} h_{x x}+\frac{B_o}{C_a} h\right] s_t \\& +\frac{1}{\gamma} \int f s_t+\frac{1}{C_a} \int\left(h_x s_x\right)_t\end{aligned}\\&\begin{aligned}=-\frac{1}{3} \int h^3 \mu_x^2 & -\frac{1}{\gamma} \int s_t^2+\int\left(\frac{1}{C_a} s_{xx}+\frac{B_o}{C_a} s\right) h_t+\int\left(\frac{1}{C_a} h_{x x}+\frac{B_o}{C_a} h\right) s_t \\& +\frac{1}{\gamma} \int f s_t+\frac{1}{C_a}\left(h_x s_x\right)_t\end{aligned}\end{aligned}\end{equation}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}
